Arrival Time Distributions of Spin-1/2 Particles

The arrival time statistics of spin-1/2 particles governed by Pauli's equation, and defined by their Bohmian trajectories, show unexpected and very well articulated features. Comparison with other proposed statistics of arrival times that arise from either the usual (convective) quantum flux or from semiclassical considerations suggest testing the notable deviations in an arrival time experiment, thereby probing the predictive power of Bohmian trajectories. The suggested experiment, including the preparation of the wave functions, could be done with present-day experimental technology.

==> letter_to_experimentalists_.tex <==
Proposal for a quantum mechanical arrival time measurement for spin-1/2 particles

Dear Dr. Steinberg,

We seek your opinion on a suggested experiment for measuring the arrival times of spin 1/2 particles (see attachment), which shows (in a Bohmian treatment) rather astonishing and significant behavior.

Briefly, we propose the measurement of arrival times of a spin-1/2 particle propagating in a cylindrical waveguide. Our analysis indicates that, depending on the initial wave function (a ground state of the particle in the cylinder), the arrival time statistics show very surprising behavior. In particular, an intriguing spin dependence manifests, hitherto unknown, with measurable consequences.

The experiment, including the preparation of the initial wave functions, can be done with present-day technology. It could become the first serious arrival time measurement, which would not only be INEXPLICABLE in terms of semiclassical (time of flight) ideas, but also serve as a benchmark for attempts to predict arrival times in quantum mechanics. A more detailed analysis of the experiment (involving Paul traps) and a fully analytic treatment of our proposal are in preparation and will soon be released. We would be very appreciative if you could refer our work to colleagues who might be interested in performing the experiment, and to any comments, critiques, etc., of the same.

Kind regards
Siddhant Das & Detlef Dürr

duerr@mathematik.uni-muenchen.de
